Investigating the Role of Centering Theory in the Context of Neural Coreference Resolution Systems

Centering theory (CT; Grosz et al., 1995) provides a linguistic analysis of the structure of discourse. According to the theory, local coherence of discourse arises from the manner and extent to which successive utterances make reference to the same entities. In this paper, we investigate the connection between centering theory and modern coreference resolution systems. We provide an operationalization of centering and systematically investigate if neural coreference resolvers adhere to the rules of centering theory by defining various discourse metrics and developing a search-based methodology. Our information-theoretic analysis reveals a positive dependence between coreference and centering; but also shows that high-quality neural coreference resolvers may not benefit much from explicitly modeling centering ideas. Our analysis further shows that contextualized embeddings contain much of the coherence information, which helps explain why CT can only provide little gains to modern neural coreference resolvers which make use of pretrained representations. Finally, we discuss factors that contribute to coreference which are not modeled by CT such as world knowledge and recency bias. We formulate a version of CT that also models recency and show that it captures coreference information better compared to vanilla CT.

==> files/OLD_CT_formulation.tex <==
{\color{blue} 
There are two desiderata for this section.
We want to define the relevant notions in centering theory concretely and have a well-defined weighting function, e.g. below. Then,
for the remainder of the paper, we can get away with this clean abstraction.
\begin{align}
     \bCf(\Un) = \{c_1, c_2, \ldots \} \\
     w(c_n) \text{is well defined}
\end{align}
}

\subsection{OLD!!!!}
% \defn{} for the term

% \Ryan{TODO: Write out in bullet points (perhaps using itemize?) what the terms are that you want to introduce and what their symbols are. Then, once you a list, turn it into a series of short, declarative sentences.)}

% mathcal for set
% bold for order set (vector)
% normal letters for utterance
% mathfrak for document

We consider a corpus of $N$ discourse domains \ryan{Should we keep this and bold it?} $\mathcal{D} = \{D_1, \ldots, D_N\}$ which we associate with the first $N$ integers. \ryan{Does the order matter here? Is it really a set?}
a set of candidate mention spans\ryan{We didn't define span} $\mathcal{M}_i$ is to be considered for each discourse $i$.\ryan{What is a candidate mention span? This isn't clear}
The $i$-th discourse $\discourse_i= [U_1, U_2, \ldots, U_{|\discourse_i|}$],\ryan{What is the relationship between $\mathcal{D}$ and $\discourse_i$?} where $U_j$ denotes an utterance (the basic unit in centering theory, e.g. a sentence or a finite clause).\ryan{Change little $i$ to little $n$}
%
$\mathcal{M}(U_j) = \{ m_1, \ldots, m_p \} $ denotes a set of mention spans which appears in $U_j$, i.e. ($\mathcal{M}(U_j) \in \mathcal{M}_i$),
where $m_j=\langle s_j, e_j \rangle$ is a span with a start position $s_j$ and an end position $e_j$.
%
Each discourse $\mathcal{D}_{i}$ contain a set of entities $\mathcal{E}_{i} = \{e_1, e_2, \ldots, e_{|\mathcal{E}_{i}|}\}$. 
% The set of possible assignments for each $E_i$ is $f(i) = \bigcup_{i=1}^{|\mathcal{D}|}{\mathcal{M}_i}$.

Next, we introduce a mention-entity mapping function $f: \mathbb{N} \times \mathbb{N}  \mapsto \mathbb{N}$, which maps mentions $m$ to entities $e$. \ryan{Should these be sub scripted?}
The range of $f$ includes an extra value $\varepsilon$\ryan{I would like to use use $\varepsilon$ if possible} representing ``not a entity''. 
It can be instantiated by the entity linking component in end-to-end coreference model. CT also states some constraints on this function.\ryan{I don't fully understand this sentence.}
We also introduce a mention-ranking function $\pi: \mathbb{N}^p \mapsto \mathbb{N}^p$,\ryan{The typing is weird. It's a ``forced conversion'' to tuples of $p$ natural numbers. I would rather omit the types} which maps a set of mentions $\mathcal{M}(U_j)$ of size $p$ to an ordered set $\mathbf{M}(U_j)$ of the same size, given a utterance $U_j$. The ranking can be any function of $\mathcal{M}(U_j)$ and $U_j$.
The mention-ranking function has been modeled in many past works in coreference resolution \cite{Rahman:11,clark-manning-2016-deep}.
CT also places some constraints on $\pi$ such as preference for pronouns~\cite{gordon1993pronouns}, grammatical roles~\cite{grosz-etal-1995-centering} or semantic roles~~\cite{kong-etal-2009-employing}.


\paragraph{The list of forward-looking centers} is defined as an ordered set of entities corresponding to utterance $U_j$, where the set of possible assignments for each $e \in \mathbf{C_f}(U_j)$ is $f(\mathbf{M}(U_j))$.\ryan{This is a bit unclear.} 
From the perspective of CT, this corresponds to Sidner's notion of ``potential discourse foci''~\cite{sidner1979towards}. Intuitively, $\mathbf{C_f}(U_j)$\ryan{Should be bolded? And needs a $U_j$ as an argument?} is a list of important entities in the current utterance and it gets updated after every utterance. $\mathbf{C_f}(U_j)$\ryan{Why is this no longer bolded? What does bolding mean?} depend only on the expressions that constitute that utterance; they are not constrained by features of any previous utterance in the segment.
Recent entity tracking and \incremental\ coreference models \cite{liu-etal-2019-referential,toshniwal2020petra,xia-etal-2020-\incremental} model $C_f$'s for coreference resolution.

The key difference between CT and coreference resolution is in the decision function that maps mentions to entities. While coreference models define a ranking or a classification function, CT defines a set of rules and constraints on the decision. CT goes on to define:

\paragraph{The preferred center} $C_p(U_j)$ is the highest-ranked element of the CF list, i.e. $\left[\mathbf{C_f}(U_j)\right]_1$. Intuitively, this denotes the most prominent discourse foci in $U_j$, e.g. $[\mathrm{John}]_i$ in $U_1$ in \Cref{example}.
%The prediction layer of ranking as well as \incremental coreference models model the preferred center.

\paragraph{The backward-looking center} 

\begin{equation}
    \Cb(\Uj) \defeq \argmax \bCf (\Ujprev)
\end{equation}
where the $\argmax$ inspects the second elements of pair, i.e. the weight. \ryan{Would this work?}

$C_b(U_j)$ is the most highly ranked element of $\mathbf{C}_{f}(U_{j-1})$ that is realized in $U_j$. 
The definition of \textit{realize} is that $U$ is an utterance of some phrase for which center $c$ is the semantic interpretation, e.g. “the 44th US president” directly realizes “Barack Obama”.\footnote{For the formal definition of \textit{realization}, please refer to Appendix A.}
In \Cref{example}, $[\mathrm{John}]_i$ as $\left[\mathbf{C_f}(U_3)\right]_1$ appears in $\mathbf{C_f}(U_4)$, so $C_b(U_4)$ is $[\mathrm{John}]_i$; otherwise, we will look at $\left[\mathbf{C_f}(U_3)\right]_2$ and so on.
The connection between the backward-looking center and the preferred center forms the theory's key claims about coherence.




==> files/OLD_Minimizing-CT-violations-as-Regularizer.tex <==
\subsection{OLD the connection between Centering and Coreference}
CT, which is an approach to modeling certain aspects of local coherence in discourse, includes within it the component that models coreference resolution.  CT utilizes this preference for the “center of attention” to continue over successive utterances. The relative preference of the “actor focus” as the next center of attention is also captured with the “preferred center” in CT. The entities in the focus space are possible antecedents. 
Many linguistics-based approaches for coreference resolution leverage differences in coherence result from changes in the center of attention, captured by the Centering transitions and transition ordering, and from the different expressions in which centers are realized.
However, CT itself is not a theory of coreference resolution. 
\eleanor{
See Section 3 in \url{https://drive.google.com/file/d/1XV80k-uOWuSHqkS9_CH9h8xtTPcZyzkZ/view?usp=sharing}.
}

\subsection{Minimizing CT violations as Regularizer}
Let $\bm{A} = [A_{1,1}, A_{1,2}, \dots, A_{S, N}]$ be the latent variable. Let $\bm{A}_i = [A_{i,1}, A_{i,2}, \dots, A_{i, N}]$ be the latent variables corresponding to the i-th utterance.
\begin{equation}
\begin{aligned}
    &\mathbf{P}(\bm{A}_1, \ldots , \bm{A}_N| \mathcal{D}) = \prod_{i=1}^{N} \prod_{j=1}^{|\mathcal{M}_i|} \mathbf{P}(\bm{a}_{i,j}| \discourse_i) \\
    &= \prod_{i=1}^{N} \prod_{j=1}^{|\mathcal{M}_i|} \frac{expscore(\bm{a}_{i,j}, emb(i,j))}{\sum_{\bm{a}' \in \mathcal{A}_{i,j}} expscore(\bm{a}', emb(i,j))}.
\end{aligned}
    \notag
\end{equation}


The parameter learning is done by maximizing the log-likelihood of all optimal clusterings implied by the centering theory.

\begin{equation}
    \sum_{t=1}^{|D|} (\log \mathbf{P}(\bm{\hat{a}} | \mathcal{D}) - \log \sum_{\bm{a}\in \bf{\mathcal{A}}} \mathbf{P}(\bm{a} | \mathcal{D})).
    \notag
\end{equation}

where $\bm{\hat{a}}$ given $\mathcal{M}$ is computed according to Centering rules.

Define the coherence score of $\bm{a}$ as:

\begin{equation}
    s_{coh}(\bm{a}) = \sum_{i=1}^{S-1} \overline{vio}(\bm{a}_i, \bm{a}_{i+1})
    \notag
\end{equation}

where $\overline{vio}(\bm{a}_i, \bm{a}_{i+1})$ means the transition from the i-th utterance to the (i+1)-th utterance does not violate the centering rules.

Recall the Centering rules: we prefer those clusterings that provide fewer centering shifts. Formally, that is:

\begin{equation}
    CB(U_n) = CB(U_{n-1})
    \notag
\end{equation}

\begin{equation}
    CB(U_n) = CP(U_n)
    \notag
\end{equation}

Now we describe the algorithm of finding the highest-scoring clustering $\bm{a}$.

\begin{enumerate}
  \item For every utterance i in the given $\mathcal{D}$, order the mention set $\mathcal{M}_i$ by the permutation function $\pi_r: \{1, \cdots, m\} \mapsto \{1, \cdots, m\}$.
  \item Backward Dynamic Programming  
\end{enumerate}


Then we assign $\bm{\hat{a}}$ to the highest-scoring clustering $\bm{a}$.


==> files/gold_cluster_grl_table_1.tex <==
\begin{table*}[!thpb]
    \centering \small
    \begin{tabular}{c|c|c|c|c|c|c|c|c|c|c}
    \toprule[2pt]
      &  \#valid\_u&  \#nocb&  \#Cheap& \#Coh. & \#Sal. & \#Cont. & \#Ret.   & \#SShift & \#RShift & \#KP \\
    \midrule[1pt]
mean & 21.47 & 7.63 & 9.87 & 10.45 & 9.64 & 7.39 & 3.07 & 2.26 & 7.77 & 10.95\\ 
std & 18.22 & 6.40 & 10.16 & 10.12 & 9.58 & 7.51 & 3.36 & 2.75 & 7.13 & 10.74\\ 
min & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00\\ 
25\% & 7.00 & 2.00 & 2.00 & 3.00 & 3.00 & 2.00 & 1.00 & 0.00 & 2.00 & 3.00\\ 
50\% & 15.00 & 6.00 & 6.00 & 7.00 & 6.00 & 5.00 & 2.00 & 1.00 & 6.00 & 7.00\\ 
75\% & 31.25 & 11.00 & 14.00 & 15.00 & 14.00 & 11.00 & 5.00 & 3.00 & 12.00 & 15.25\\ 
max & 92.00 & 31.00 & 63.00 & 57.00 & 54.00 & 39.00 & 19.00 & 16.00 & 32.00 & 63.50\\ 
\midrule[1pt]
 & \%valid\_u & \%$\overline{nocb}$ & \%Cheap & \%Coh. & \%Sal. & \%Cont. & \%Ret. & \%SShift & \%RShift & \%KP \\ 
\midrule[1pt]
mean & 80.02 & 60.14 & 42.78 & 46.51 & 42.85 & 39.17 & 14.15 & 9.99 & 36.12 & 48.07\\ 
std & 19.26 & 17.48 & 17.57 & 15.25 & 16.05 & 23.68 & 12.46 & 10.22 & 20.02 & 14.80\\ 
min & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00\\ 
25\% & 70.00 & 50.00 & 32.71 & 37.06 & 33.33 & 24.76 & 4.17 & 0.00 & 25.00 & 39.48\\ 
50\% & 84.62 & 61.45 & 44.44 & 47.11 & 44.44 & 35.56 & 12.50 & 9.09 & 36.36 & 50.00\\ 
75\% & 95.06 & 73.08 & 53.67 & 54.96 & 52.17 & 50.00 & 20.00 & 14.85 & 50.00 & 57.54\\ 
max & 100.00 & 93.48 & 87.50 & 87.50 & 87.50 & 100.00 & 100.00 & 50.00 & 100.00 & 87.50\\ 
\bottomrule[2pt]
\end{tabular}
\caption{The detailed statistics of centering metrics on OntoNotes, with \cfCandidate\ being \clusterOnly\ and the weighting function $w$ being \grammaticalRole.}
\label{tab:gold_cluster_grl_table_1}
\end{table*}

\begin{table*}
    \centering  \small
    \begin{tabular}{c|c|c|c|c|c|c|c|c|c|c}
    \midrule[1pt]
 & \#valid\_u & \#nocb & \#Cheap & \#Coh. & \#Sal. & \#Cont. & \#Ret. & \#SShift & \#RShift & \#KP \\ 
    \toprule[2pt]
mean & 21.47 & 7.63 & 9.60 & 10.22 & 8.79 & 6.68 & 3.54 & 2.10 & 8.15 & 10.61\\ 
std & 18.22 & 6.40 & 9.86 & 9.88 & 8.67 & 6.83 & 3.82 & 2.52 & 7.46 & 10.36\\ 
min & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00\\ 
25\% & 7.00 & 2.00 & 2.75 & 3.00 & 2.00 & 2.00 & 1.00 & 0.00 & 2.00 & 3.00\\ 
50\% & 15.00 & 6.00 & 6.00 & 7.00 & 6.00 & 4.00 & 2.00 & 1.00 & 6.00 & 6.75\\ 
75\% & 31.25 & 11.00 & 14.00 & 15.00 & 13.00 & 10.00 & 5.00 & 3.00 & 13.00 & 15.56\\ 
max & 92.00 & 31.00 & 60.00 & 60.00 & 52.00 & 42.00 & 18.00 & 12.00 & 32.00 & 63.00\\ \midrule[1pt]
  & \%valid\_u & $\textrm{\%}\overline{\textrm{nocb}}$ & \%Cheap & \%Coh. & \%Sal. & \%Cont. & \%Ret. & \%SShift & \%RShift & \%KP \\ 
\midrule[1pt]
mean & 80.02 & 60.14 & 41.62 & 45.79 & 39.67 & 36.50 & 16.10 & 9.23 & 37.59 & 46.81\\ 
std & 19.26 & 17.48 & 17.03 & 14.75 & 15.64 & 23.93 & 13.34 & 9.44 & 19.86 & 14.10\\ 
min & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & -0.00 & 0.00\\ 
25\% & 70.00 & 50.00 & 30.19 & 36.09 & 29.45 & 22.22 & 7.55 & 0.00 & 25.82 & 38.65\\ 
50\% & 84.62 & 61.45 & 42.86 & 46.15 & 40.00 & 33.33 & 15.38 & 8.33 & 38.46 & 47.79\\ 
75\% & 95.06 & 73.08 & 52.50 & 54.17 & 50.00 & 46.15 & 23.08 & 14.29 & 50.00 & 56.51\\ 
max & 100.00 & 93.48 & 80.00 & 85.71 & 80.00 & 100.00 & 100.00 & 50.00 & 100.00 & 80.00\\ 
    \bottomrule[2pt]
    \end{tabular}
\caption{The detailed statistics of centering metrics on OntoNotes, with \cfCandidate\ being \clusterOnly\ and the weighting function being \semanticRole.}
\label{tab:best_cluster_srl_table_1}
\end{table*}


==> files/intro_stash.tex <==
\section{Old Introduction}
% ada tta bilità
% ada pta bility 
%%%% Centering theory~\cite{grosz-etal-1995-centering} is the best-known framework for theorizing about local coherence and salience. It is widely used in the literature of coreference resolution in the 20-th century and the first decade of this century, e.g. \cite{brennan-etal-1987-centering}, \cite{sidner1979towards}, \cite{beaver2004optimization},  \cite{kong-etal-2009-employing}.
%%%% Our main goal is to investigate if modern coreference resolution algorithms follow the constraints and rules laid out by centering theory~\cite{grosz-etal-1995-centering} and its follow-ups~\cite{poesio-etal-2004-centering}.

\ryan{We need a better inroductory papergraph. The purpose of this first paragraph is two take two disparate lines of research and convince the reader that they should be unified or, at least, discussed in the same context. Instead, it provides a super short overview of center theory. A topical sentence about the entire paper would help.}

Centering theory~\cite{grosz-etal-1995-centering} has served as the theoretical foundation for a lot of work in discourse analysis. 
Centering describes the notion of \textbf{local coherence} in natural language text through modeling the relationship between discourse entities and their references. 
%by characterizing entity-level coherence, concerning the way \textit{centers} (or discourse entities and their referents), %such as named entities and possessive pronouns, 
%are introduced and subsequently discussed.

Coreference resolution, on the other hand, is the process of linking
various referring expressions of a given entity in the text.\ryan{This feels like an abrupt change. I expected the text to discuss coreference NLP, but we jump to psycholinguistics.}
%The key in coreference resolution is to determine the antecedent for each referring expression in a text. %Coreference also accounts for coherence and cohesion in a text.
It has been claimed in previous psycholinguistic literature~\cite{chambers1998structural, gordon1998representation} that there is a connection between coreference and centering theory. \ryan{This is the first connection the two, but this would have been confusing to me if I didn't know what the paper was about.} This connection has also been explored in subsequent NLP literature. 
Algorithms based on centering theory have been often cited and used in coreference resolution literature ~\cite{brennan-etal-1987-centering, sidner1979towards, iida2003incorporating, beaver2004optimization, kong-etal-2009-employing}.
Some early works claimed that the constraints
proposed by the theory can be useful to guide coreference resolution~\cite{elango2005coreference, deemter2000coreferring}.
However, some more recent works \cite{yang2004improving} have also called this into question and have shown that the use of these constraints fails to improve or even harms the performance of coreference resolution systems. 

% no need for new paragraph
% Both \citep and \citet are defined by natbib and are thus not standard. The standard LaTeX command \cite should be avoided, because it behaves like \citet for author-year citations, but like \citep for numerical ones. There are many other commands for other special effects (Section 2.4).
\ryan{I think this paragraph wants to say that we should use modern neural coreference systems to test parts of centering theory!}
As neural networks have regained popularity, end-to-end neural approaches ~\cite{lee-etal-2017-end, joshi-etal-2019-bert} have become the main building-block of modern coreference resolution systems.
However, the questions: \textbf{(a) to what extent do these approaches model discourse structure in text}, \textbf{(b) to what extent do these models follow the principles of centering theory}, and \textbf{(c) can these models further benefit from an improved modelling of discourse structure} remain unexplored.

The goal of this paper is to answer the above questions in the context of modern end-to-end coreference resolution systems.
%by centering theory and its follow-ups~\cite{poesio-etal-2004-centering}. 
We answer these questions by carefully analyzing these coreference models based on discourse information and conducting appropriate statistical tests.
%, in which the role of other factors is deliberately ignored.
Since centering theory is a linguistic theory and not a computational one, this first requires operationalizing centering theory, that is, building a computational CT framework. This requires defining the various undefined parameters in the original centering theory \cite{grosz-etal-1995-centering}.
%compatible with modern coreference resolution models. We then reformulate and implement the state-of-the-art resolution model in this framework~\cite{lee-etal-2017-end, joshi-etal-2020-spanbert}. The evaluation is carried out by an appropriate method (and various statistical tests): 
Then, we adopt a search-based procedure \cite{karamanis2004evaluating} on the outputs of these coreference resolution models and randomly shuffle the orderings of utterances in a specific discourse
%and evaluate them according 
to compute 
%scores assigned by 
various center-based metrics described in previous works \cite{poesio-etal-2004-centering}. The assumption behind these mentrics is that the best-scoring ordering among the candidate orderings should be the original ordering.
Then, we conduct experiments establishing a positive correlation between the centering metrics and coreference model performance.
%These experiments reveal that there is indeed a positive correlation between the centering metrics and 
We further explore the space of parameter configurations of CT using modern natural language processing techniques, measuring the impact of different ways of setting the parameters, choice of different pretrained embeddings and verifying the robustness of our analytical results. 


By a series of systematic analyses, we show that 1) state-of-the-art coreference resolution models achieve relatively high scores assigned by center-based metrics, indicating they do contain some information about discourse-level entity coherence, even though they are not trained by any CT signals; 2) there is a positive dependence between coref F1 and center-based metrics, verifying the psycholinguistic claim about coreference and CT; 3) the scores of center-based metrics converge as coref F1 increase: the dependence between them decreases when CoNLL F1 score reaches above 55\%, however, this interval is where all modern coreference resolution models lie. This, to some extent, indicates that the current improvements in coreference resolution performance no longer improve entity-coherence. We also show that contextualized embeddings contain much coherence information by information-theoretic analysis, which helps explain why little gains can CT provide to SOTA coreference models.

The article is organized as follows. Section \ref{ct} briefly describes some related work. We then summarize the basic concepts of CT in Section 3. Section 4 proposes a general centering framework of coreference and coherence. 
Section 6 details the analysis methodology. In Section 7 and 8 we present our experimental results and analysis, which are discussed in Section 9.

==> files/stash01.tex <==
\subsection{Coherence Modeling}
Coherence Modeling for the Automated Assessment of Spontaneous Spoken Responses~\cite{wang-etal-2013-coherence}:
They investigate the use of several features originally developed for essays (entity Grid and e-rater Features) to model coherence in spoken responses. An analysis on an annotated corpus shows that the prediction accuracy for human holistic scores of an automated speech scoring system can be improved by around 10\% relative after the addition of the coherence features.  Further experiments indicate that a weighted F-Measure of 73\% can be achieved for the automated prediction of the coherence scores. (this study treats coherence prediction as a binary classification task: low-coherent vs. high-coherent, where the low-coherent responses are those with average scores 1 and 1.5, and the high-coherent responses are those with average scores 2, 2.5, and 3)

Towards enabling feedback on rhetorical structure with neural sequence models~\cite{10.1145/3303772.3303808}: 


\subsection{Automated Essay Scoring}
A Neural Approach to Automated Essay Scoring~\cite{taghipour-ng-2016-neural}: 
An early deep learning approach using a
combination CNN+LSTM architecture that
outperformed most reported results at that
time.


Automated essay scoring with discourse-aware neural models~\cite{nadeem-etal-2019-automated}: explores network structures, contextualized embeddings and pre-training strategies aimed at capturing discourse characteristics of essays. Experiments on three essay scoring tasks show benefits from all three strategies in different combinations, with simpler architectures being more effective when less training data is available.

Language models and automated
essay scoring~\cite{rodriguez2019language}: exploratory studies that attempts AES with a variety of pretrained neural models, including BERT and XLNet, with numerous alternate conﬁgurations and training methods (arkiv).


Should You Fine-Tune BERT for Automated Essay Scoring?~\cite{mayfield-black-2020-fine}:
They argue that while state-of-the-art strategies do match existing best results, they come with opportunity costs in computational resources. They conclude with a review of promising areas for research on student essays where the unique characteristics of Transformers may provide beneﬁts over classical methods to justify the costs.

\subsubsection{NLP for Automated Essay Scoring}
\paragraph{Representations}
\begin{itemize}
    \item Bag-of-Words Representations: N-grams based on part-of-speech tags (of length 2-3) to capture syntax independent of content, and character-level N-grams of length 3-4, to provide robustness to misspellings
    \item Word Embeddings
    \item Fine-Tuning BERT
    \item Feature Extraction from BERT: the embedding of [CLS].
\end{itemize}

\paragraph{Metrics}
The standard metric for measuring reliability of automated assessments in the AES community: a variant of Cohen’s kappa, with quadratic weights for “near-miss” predictions on an ordinal scale (QWK). 

\paragraph{Baselines}
\begin{itemize}
    \item Human IRR
    \item Industry best performance
    \item \cite{taghipour-ng-2016-neural}
    \item Two recent results using traditional non-neural models: \citet{woods2017formative}, which uses n-gram features in an ordinal logistic regression, and \citet{cozma-etal-2018-automated}, which uses a mix of string kernels and word2vec embeddings in a support vector regression.
    \item \cite{rodriguez2019language}
\end{itemize}

\subsubsection{The SOTA Implementation~\cite{woods2017formative}}
Turned out to be an non-neural method!
They propose to combine string kernels (low-level character n-gram features) and word embeddings (high-level semantic features) for automated essay scoring (AED).

\paragraph{String Kernels} The histogram intersection string kernel (HISK),

\paragraph{Bag-of-Super-Word-Embeddings}
\begin{enumerate}
    \item Each word in the collection of documents is represented as word vector using a pre-trained word embeddings model.
    \item Clustering
    \item Every embedded word in the collection of documents is then assigned to the nearest cluster centroid(the nearest super word vector).
    \item the super word vectors generate a vocabulary (codebook)
    \item represent each document as a bag-of-super-word-embeddings (BOSWE) using that codebook (compute the occurrence count of each super word embedding in the respective document).
\end{enumerate}


\paragraph{Learning}
After getting vector representations of documents, thet employ $v$-Support Vector Regression ($v$-SVR) in order to automatically predict the score for an essay. 
They fussion two parts by simply summing up the two corresponding kernel matrices (equivalent to feature vector concatenation in the primal Hilbert space)

No order (no coherence information in it).


\subsubsection{Summary of AED}
ASAP is a supervised regression problem. They only care about how similar the documents of the same level are, rather than eveluating different aspects of text quality (e.g. coherence, vocabulary...).

In contrast, we focus on unsupervised/weakly-supervised AED. 









\section{Naive Metrics}
\textbf{Given a sequence of $C_f$-lists}, the statistics about transitions computed as just discussed can be used to determine the degree to which a text conforms with, or violates, Centering’s principles. Here are 4 naive statistical measurements:

\textbf{M.NOCBS} is to classify each ordering of propositions according to the number of NOCBs it contains, and pick the ordering with the fewest NOCBs ($C_b(U_{n-1})$ is undefined, which implies no element in $C_f(U_{n-1})$ is realized in $U_n$).

\textbf{M.CHEAP} is biased in favour of the ordering with the fewest violations of CHEAPNESS ($C_b(U_n)=C_p(U_{n−1})$).

\textbf{M.KP} sums up the NOCBs and the violations of CHEAPNESS, COHERENCE ($C_b(U_n)=C_b(U_{n−1})$) and SALIENCE ($C_b(U_n)=C_p(U_n)$), preferring the ordering with the lowest total cost (Kibble and Power, 2000). 

\textbf{M.BFP} employs the preferences between standard transitions as expressed by Rule 2.

\textbf{But how to get $C_f$-lists?}

\section{Possible Mathematical Tools}
\begin{itemize}
    \item A better $P(\bm{C}_f \mid \bm{D})$: CRF for selecting and ranking Cf-list
    \item formulate ILP constrains
    \item The Dempster--Shafer Decision Model
    \item Add an extra causal link: $$P(\bm{C}, \bm{C_f} \mid \bm{D}) = P(\bm{C_f} \mid \bm{D})P(\bm{C} \mid \bm{C_f},\bm{D} )$$
\end{itemize}

\section{Coherence Modeling}
\subsection{Definitions}
Let $\bm{C}$ denotes the random variable of coherence. $\bm{D}= [U_1, U_2, \ldots, U_{|\bm{D}|}$] denotes the discourse being evaluated, and utterance 
$U = [u_1, u_2, \ldots, u_{|U|}]$ denotes a sequence of tokens.\ryan{What sort of tokens? What are they tokens of?}. let $M = \langle m_1, \ldots, m_p \rangle $ denote a mention set of $U$, where $m_j=\langle s_j, e_j \rangle$ is a span with a start position $s_j$ and an end position $e_j$. Each discourse $\bm{D}$ comes with a set of entities $\bm{E} = \{E_1, E_2, \ldots, E_{|\bm{E}|}\}$, where an entity $E_i$ is a special span. The set of possible assignments for each $E_i$ is $\mathcal{E}(i) = \bigcup_{i=1}^{|\bm{D}|}{\bm{M}_i}$. $\bm{C_f}_i = [E_{i_1}, E_{i_2}, \ldots, E_{i_{|\bm{C_f}_i|}}]$ is an ordered set of entities corresponding to utterance $U_i$, where the set of possible assignments for each $E_{i_j}$ is $\bm{M}_i \cap \bm{E} \cup \{ \epsilon \} $. $\epsilon$ is a dummy head. 

Coherence measuring in \citet{karamanis2004evaluating} is actually:
\begin{equation}
p(\bm{C}, \bm{C_f} \mid \bm{D}) = p(\bm{C_f} \mid \bm{D})\,p(\bm{C} \mid \bm{C_f})
\end{equation}
where $p(\bm{C_f} \mid \bm{D})$ denotes the process of mention detection, mention pruning and entity ranking.






\section{Datasets}
\subsection{ASAP}
5 datasets from the ASAP competition, jointly hosted by the Hewlett Foundation and Kaggle.com~\cite{perelman2014state}.

\subsection{Spoken responses from TOEFL}
used in \citet{wang-etal-2013-coherence}. They collected 600 spoken responses from the international TOEFL® iBT assessment of English proficiency for non-native speakers.

\begin{table*}[hpb]
\centering  
\begin{tabular}{c|c|c|c|c|c}
\toprule[2pt]
 & \%valid\_u & \#nocb & \#Cheap & \#Coh. & \#Sal.\\ 
\midrule[1pt]
Seman. & 17.20 (16.42) & 6.01 (5.57) & 8.12 (9.64) & 8.23 (9.17) & 7.67 (8.68) & 5.75 (6.57) & 2.47 (3.23) & 1.92 (2.81) & 6.07 (6.28) & 8.80 (9.97) \\ 
 & 79.48(21.20) & 59.31(19.09) & 43.15(18.41) & 45.04(16.06) & 41.90(16.62) & 39.79(25.86) & 13.78(13.24) & 10.22(11.86) & 35.27(22.09) & 47.35(15.32) \\ 
\bottomrule[2pt]
\end{tabular}
\caption{The Detailed Statistics of CT-based metrics on OntoNotes, with CF candidates being ``cluster only'' and CF ranking being semantic-role-based.}
\label{tab:statistics}
\end{table*}


\subsection{Minimizing CT violations as Regularizer}
\eleanor{this part is irrelevant in this analysis paper}
\mrinmaya{We can comment it out}
Let $\bm{A} = [A_{1,1}, A_{1,2}, \dots, A_{S, N}]$ be the latent variable. Let $\bm{A}_i = [A_{i,1}, A_{i,2}, \dots, A_{i, N}]$ be the latent variables corresponding to the i-th utterance.
\begin{equation}
\begin{aligned}
    &\mathbb{P}(\bm{A}_1, \ldots , \bm{A}_N| \mathcal{D}) = \prod_{i=1}^{N} \prod_{j=1}^{|\mathcal{M}_i|} \mathbb{P}(\bm{a}_{i,j}| \mathcal{D}_i) \\
    &= \prod_{i=1}^{N} \prod_{j=1}^{|\mathcal{M}_i|} \frac{expscore(\bm{a}_{i,j}, emb(i,j))}{\sum_{\bm{a}' \in \mathcal{A}_{i,j}} expscore(\bm{a}', emb(i,j))}.
\end{aligned}
    \notag
\end{equation}


The parameter learning is done by maximizing the log-likelihood of all optimal clusterings implied by the centering theory.

\begin{equation}
    \sum_{t=1}^{|D|} (\log \mathbb{P}(\bm{\hat{a}} | \mathcal{D}) - \log \sum_{\bm{a}\in \bf{\mathcal{A}}} \mathbb{P}(\bm{a} | \mathcal{D})).
    \notag
\end{equation}

where $\bm{\hat{a}}$ given $\mathcal{M}$ is computed according to Centering rules.

Define the coherence score of $\bm{a}$ as:

\begin{equation}
    s_{coh}(\bm{a}) = \sum_{i=1}^{S-1} \overline{vio}(\bm{a}_i, \bm{a}_{i+1})
    \notag
\end{equation}

where $\overline{vio}(\bm{a}_i, \bm{a}_{i+1})$ means the transition from the i-th utterance to the (i+1)-th utterance does not violate the centering rules.

Recall the Centering rules: we prefer those clusterings that provide fewer centering shifts. Formally, that is:

\begin{equation}
    CB(U_n) = CB(U_{n-1})
    \notag
\end{equation}

\begin{equation}
    CB(U_n) = CP(U_n)
    \notag
\end{equation}

Now we describe the algorithm of finding the highest-scoring clustering $\bm{a}$.

\begin{enumerate}
  \item For every utterance i in the given $\mathcal{D}$, order the mention set $\mathcal{M}_i$ by the permutation function $\pi_r: \{1, \cdots, m\} \mapsto \{1, \cdots, m\}$.
  \item Backward Dynamic Programming  
\end{enumerate}


Then we assign $\bm{\hat{a}}$ to the highest-scoring clustering $\bm{a}$.


==> tabs/correlation.tex <==
\begin{table*}
\centering \footnotesize
\begin{tabular}{c|cc|cc||cc|cc|cc}
\toprule[2pt]
       &  \multicolumn{2}{c}{All} & \multicolumn{2}{c}{SOTAs} &  \multicolumn{2}{c}{SpanBERT} & \multicolumn{2}{c}{GloVe}  & \multicolumn{2}{c}{One-hot}\\
\textbf{Metric}   & Cor. & MI  & Cor. & MI   & Cor. & MI  & Cor. & MI & Cor. & MI\\
\midrule[1pt]
\textsc{$\lnot$nocb}	&	0.882$\dag$	& 0.456 & 0.521$\dag$ & 1.06e-3	&	0.903$\dag$	& 0.341 & 0.939$\dag$ & 0.788 & 0.846$\dag$ & 0.504 \\
\textsc{cheap} 	&	0.858$\dag$	& 0.384 & -0.191$\dag$ & 3.52e-2&	0.872$\dag$	& 0.120 & 0.929$\dag$ & 0.684 & 0.837$\dag$ & 0.481\\
\textsc{coherence} 	&  0.864$\dag$ & 0.346 & -0.026 & 3.52e-2&  0.871$\dag$ & 0.134 & 0.934$\dag$  & 0.650 & 0.837$\dag$ & 0.452\\
\textsc{salience} 	&0.897$\dag$ & 0.490 & 0.802$\dag$ & 6.73e-2& 0.913$\dag$ & 0.382 & 0.942$\dag$ & 0.777 & 0.850$\dag$ & 0.492\\
\textsc{kp}    	& 0.883$\dag$ & 0.451 & 0.459$\dag$ & 1.49e-3	& 0.903$\dag$ & 0.324 & 0.941$\dag$ & 0.796 & 0.858$\dag$ & 0.542\\
\textsc{transition} 	&	0.912$\dag$ & 0.296 & 0.477$\dag$ & 1.20e-2& 0.899$\dag$ & 0.211 & 0.964$\dag$ & 0.648 & 0.844$\dag$ & 0.469\\
\bottomrule[2pt]
\end{tabular}
    \caption{Pearson correlation coefficient and mutual information of CoNLL F1 with centering metrics. p-value $<0.01$ is denoted as $\dag$.}
    \label{tab:correlation}
    \vspace{-0.1in}
\end{table*}

% Table: MI/correlations
% \begin{table}[thpb]
% \centering \scriptsize
% \begin{tabular}{c|cc|cc|cc}
% \toprule[2pt]
%       &  \multicolumn{2}{|c}{SpanBERT} & \multicolumn{2}{|c}{GloVe}  & \multicolumn{2}{|c}{One-hot}\\
% \textbf{Metric}   & Cor. & MI  & Cor. & MI  & Cor. & MI\\
% \midrule[1pt]
% \textsc{$\lnot$nocb}	&	0.903$\dag$	& 0.341 & 0.939$\dag$ & 0.788 & 0.846$\dag$ & 0.504 \\
% \textsc{cheap} 	&	0.872$\dag$	& 0.120 & 0.929$\dag$ & 0.684 & 0.837$\dag$ & 0.481\\
% \textsc{coherence} 	&  0.871$\dag$ & 0.134 & 0.934$\dag$  & 0.650 & 0.837$\dag$ & 0.452\\
% \textsc{salience} 	& 0.913$\dag$ & 0.382 & 0.942$\dag$ & 0.777 & 0.850$\dag$ & 0.492\\
% \textsc{kp}    	& 0.903$\dag$ & 0.324 & 0.941$\dag$ & 0.796 & 0.858$\dag$ & 0.542\\
% \textsc{transition} 	& 0.899$\dag$ & 0.211 & 0.964$\dag$ & 0.648 & 0.844$\dag$ & 0.469\\
% \bottomrule[2pt]
% \end{tabular}
%     \caption{The Pearson correlation coefficients and mutual information of CoNLL F1 with centering metrics. p-value $<0.01$ is denoted as $\dag$.}
%     \label{tab:Glove-vs-Spanbert-Cor-MI}
%     \vspace{-0.1in}
% \end{table}

% \begin{figure}[thpb]
% % \centering
% \includegraphics[scale = 0.15]{Glove-Spanbert-onehot-Cor-MI-data.png}
% \caption{The mutual information between CoNLL F1 and centering scores as a function of the amount of coreference training data. X-axis represents the ratio of the Ontonotes dataset used in training.}
% \label{fig:Glove-vs-Spanbert-Cor-MI-data}
% \vspace{-0.1in}
% \end{figure}


==> tabs/ontonotes_stat.tex <==
\begin{table}
    \centering \small
    \begin{tabular}{c|ccc|ccc}
    \toprule[2pt]
         & \multicolumn{3}{c|}{\textit{\#Sent}} &\multicolumn{3}{c}{\textit{ \#Token}} \\
        
         & mean & min & max & mean. & min & max \\
    \midrule[1pt]
Train    & 26.83 & 1 & 188 & 463.71 & 24 & 4009\\
Dev   & 27.99 & 2 & 127 & 475.52 & 33 & 2314\\
Test & 27.24 & 2 & 140 & 487 & 34 & 1798\\
    \bottomrule[2pt]
    \end{tabular}
    \caption{The statistics of the number of sentences and the number of tokens per document of OntoNotes.}
    \label{tab:dataset_stat}
    \vspace{-0.1in}
\end{table}

==> tabs/t1_statistics.tex <==
% tab:t1_statistics
\begin{table}
\centering
\begin{adjustbox}{width=0.49\textwidth}
\begin{tabular}{c|c|c|c|c|c}
\toprule[2pt]
 & \%valid\_u & \%$\overline{\text{nocb}}$ & \%Cheap & \%Coh. & \%Sal.\\ 
\midrule[1pt]
Gram. & 80.02 & 60.14 & 42.78 & 46.51  & 42.85 \\ 
Seman. & 79.48  & 59.31& 43.15 & 45.04 & 41.90 \\
Gram.+forget &  80.02 & - \\
Seman. +forget & 79.48  &  - \\
\midrule[1pt]
 & \%Cont. & \%Ret. & \%SShift & \%RShift & \%KP \\ 
\midrule[1pt]
Gram.  & 39.17  & 14.15  & 9.99  & 36.12  & 48.07 \\ 
Seman. & 39.79 & 13.78  & 10.22  & 35.27  & 47.35  \\
Gram.+forget & 80.02 & - \\
Seman. +forget & 79.48  &  - \\
\bottomrule[2pt]
\end{tabular}
\end{adjustbox}
    \caption{Statistics of centering metrics on OntoNotes 5.0 testset. \textit{Gram.} and \textit{Seman.} stand for \grammaticalRole\ and \semanticRole\ weighting functions, respectively. +forget indicate that the forget function is adopted. \textit{valid\_u} are the valid utterances (not null utterances). \textit{\%valid\_u} represents the percentage of valid utterances. \textit{\%Cheap}, \textit{\%Coh.}, \textit{\%Sal.}, \textit{\%Cont.}, \textit{\%Ret.}, \textit{\%SShift}, and \textit{\%RShift} represent the percentage of transition that satisfy \textsc{cheap}, \textsc{coherence}, \textsc{salience}, \Continue, \Retain, \SmoothShift, \RoughShift,  respectively. \textit{\%KP} represents the average of the conditions.\looseness=-1} %\footnotemark}
\label{tab:t1_statistics}
\vspace{-0.5cm}
\end{table}
%\footnotetext{The complete statistics are listed in Appendix D.}
